Information Rates Over Multi-View Channels

We investigate the fundamental limits of reliable communication over multi-view channels, in which the channel output is comprised of a large number of independent noisy views of a transmitted symbol. We consider first the setting of multi-view discrete memoryless channels and then extend our results to general multi-view channels (using multi-letter formulas). We argue that the channel capacity and dispersion of such multi-view channels converge exponentially fast in the number of views to the entropy and varentropy of the input distribution, respectively. We identify the exact rate of convergence as the smallest Chernoff information between two conditional distributions of the output, conditioned on unequal inputs. For the special case of the deletion channel, we compute upper bounds on this Chernoff information. Finally, we present a new channel model we term the Poisson approximation channel -- of possible independent interest -- whose capacity closely approximates the capacity of the multi-view binary symmetric channel for any fixed number of views.

==> acknowledgement.tex <==
The research of NW was partially supported by the Israel Science Foundation (ISF), grant no. 1782/22.

==> appprop1.tex <==
\subsection{Proof of Proposition \ref{prop:1}}
\label{appb}
\begin{proof}
	Let $\pi\in G_\mathcal{A}$ be a permutation in the symmetry group of $\mathcal{A}$ and let $f$ be some feasible solution to $\mathsf{Del}(n,d;\mathcal{A})$.
	
	\begin{itemize}
		\item[(D1)] It is clear that if $f(\mathbf{x})\geq 0$, then $f(\pi \cdot \mathbf{x})\geq 0$, for all $\mathbf{x}\in \{0,1\}^n$.
		\item[(D2)] The fact that if $\widehat{f}(\mathbf{s})\geq 0$, then it holds that $\widehat{\pi\circ f}(\mathbf{s})\geq 0$, for all $\mathbf{s}\geq 0$, follows from the simple lemma below:
		\begin{lemma}
			\label{lem:perm}
			For any function $f: \{0,1\}^n \to \mathbb{R}$ and for any permutation $\sigma \in S_n$, it holds that
			\[
			\widehat{\sigma \circ f}(\mathbf{s}) = (\sigma \circ \widehat{f})(\mathbf{s}), \quad \text{for all $\mathbf{s}\in \{0,1\}^n$}.
			\]
		\end{lemma}
		\begin{proof}
			Observe that 
			\begin{align*}
				\widehat{\sigma \circ f}(\mathbf{s})&= \sum_{\mathbf{x}\in \{0,1\}^n} f(\sigma\cdot \mathbf{x})\cdot (-1)^{\mathbf{x}\cdot \mathbf{s}}\\
				&= \sum_{\mathbf{x}\in \{0,1\}^n} f(\sigma\cdot \mathbf{x})\cdot (-1)^{(\sigma\cdot\mathbf{x})\cdot (\sigma\cdot\mathbf{s})}\\
				&=\sum_{\mathbf{x}\in \{0,1\}^n} f(\mathbf{x})\cdot (-1)^{\mathbf{x}\cdot (\sigma\cdot\mathbf{s})}
				=  (\sigma \circ \widehat{f})(\mathbf{s}).
			\end{align*}
		\end{proof}
		\item[(D3)] Since any permutation in $G_\mathcal{A}$ also lies in $S_n$ and hence preserves the weights of vectors in $\{0,1\}^n$, it holds that $(\pi\circ f)(\mathbf{x}) = 0$, for all $\mathbf{x}\in \{0,1\}^n$ such that $1\leq w(\mathbf{x})\leq d-1$.
		\item[(D4)] This constraint is also satisfied by $\pi \circ f$, since $\pi(0^n) = 0^n$, for all $\pi\in G_\mathcal{A}$.
		\item[(D5)] Observe that for any $\pi\in G_\mathcal{A}$,
		\begin{align*}
			2^n\cdot (\mathds{1}_\mathcal{A}\star \mathds{1}_\mathcal{A})(\pi\cdot \mathbf{x})&= \sum_{\mathbf{z}\in \{0,1\}^n} \mathds{1}_\mathcal{A}(\mathbf{z})\cdot \mathds{1}_\mathcal{A}(\pi\cdot \mathbf{x}+\mathbf{z})\\
			&= \sum_{\mathbf{z}\in \{0,1\}^n} \mathds{1}_\mathcal{A}(\pi\cdot \mathbf{z})\cdot \mathds{1}_\mathcal{A}(\pi\cdot \mathbf{x}+\pi\cdot \mathbf{z})\\
			&= \sum_{\mathbf{z}\in \{0,1\}^n} \mathds{1}_\mathcal{A}(\pi\cdot \mathbf{z})\cdot \mathds{1}_\mathcal{A}(\pi\cdot (\mathbf{x}+ \mathbf{z}))\\
			&= \sum_{\mathbf{z}\in \{0,1\}^n} \mathds{1}_\mathcal{A}(\mathbf{z})\cdot \mathds{1}_\mathcal{A}(\mathbf{x}+ \mathbf{z})\\ &= 2^n\cdot (\mathds{1}_\mathcal{A}\star \mathds{1}_\mathcal{A})(\mathbf{x}).
		\end{align*}
		Hence, since for all $\mathbf{x}\in \{0,1\}^n$, we have that
		\begin{align*}
			\pi\circ f(\mathbf{x})&\leq 2^n\cdot (\mathds{1}_\mathcal{A}\star \mathds{1}_\mathcal{A})(\pi\cdot \mathbf{x})\\
			&= 2^n\cdot (\mathds{1}_\mathcal{A}\star \mathds{1}_\mathcal{A})(\mathbf{x}),
		\end{align*}
		we have that (D5) is also satisfied by $\pi\circ f$.
		\item[(Obj$^\prime$)] It is clear that $\sum_{\mathbf{x}} f(\mathbf{x}) = \sum_{\mathbf{x}} f(\pi\cdot \mathbf{x})$, and hence that val$(f) = \text{val}(\pi\circ f)$.
	\end{itemize}
\end{proof}
